TRAIL: Topology Authentication in RPL

The IPv6 Routing Protocol for Low-Power and Lossy Networks (RPL) was recently introduced as the new routing standard for the Internet of Things. Although RPL defines basic security modes, it remains vulnerable to topological attacks which facilitate blackholing, interception, and resource exhaustion. We are concerned with analyzing the corresponding threats and protecting future RPL deployments from such attacks. Our contributions are twofold. First, we analyze the state of the art, in particular the protective scheme VeRA and present two new rank order attacks as well as extensions to mitigate them. Second, we derive and evaluate TRAIL, a generic scheme for topology authentication in RPL. TRAIL solely relies on the basic assumptions of RPL that (1) the root node serves as a trust anchor and (2) each node interconnects to the root as part of a hierarchy. Using proper reachability tests, TRAIL scalably and reliably identifies any topological attacker without strong cryptographic efforts.

==> 00_grafx/formeln.tex <==

%v0 one line
$\langle V_{0}, c_{1}, R_{Sender},$
\newline
$\{V_{0}, c_{1}\}_{sign} \rangle$

%V1
$\langle V_{1}, c_{2}, R_{Sender} \rangle$

%V2
$\langle V_{2}, c_{3}, R_{Sender} \rangle$

%V3
$\langle V_{3}, c_{4}, R_{Sender} \rangle$


%Vn-1
$\langle V_{n-1}, R_{n, l},$ 
\newline
$R_{Sender} \rangle$


%Spalte rechts mit \vspace{0.03cm}j

%1 neu
$dec _{c_{2}} (c_{1}) = R_{1, l}$
\newline
$h^1(V_1) \stackrel{?}{=} V_0 ,\,  h^{l-j}(R_{Sender}) \stackrel{?}{=} R_{1,l}$


% 1
$\textrm{\footnotesize{decrypt:}\,}dec _{c_{2}} (c_{1}) = R_{1, l}$
\newline
$\textrm{\footnotesize{verify:  \,\,}\,}h^{l-j}(R_{Sender}) \stackrel{?}{=} R_{1,l}$

% 2
$\textrm{\footnotesize{decrypt:}\,}dec _{c_{3}} (c_{2}) = R_{2, l}$
\newline
$\textrm{\footnotesize{verify:  \,\,}\,}h^{l-j}(R_{Sender}) \stackrel{?}{=} R_{2,l}$

% 3
$\textrm{\footnotesize{decrypt:}\,}dec _{c_{4}} (c_{3}) = R_{3, l}$
\newline
$\textrm{\footnotesize{verify:  \,\,}\,}h^{l-j}(R_{Sender}) \stackrel{?}{=} R_{3,l}$

% n-1
$\textrm{\footnotesize{decrypt:}\,}dec _{R_{n,l}} (c_{n-1}) = R_{n-1, l}$
\newline
$\textrm{\footnotesize{verify:  \,\,}\,}h^{l-j}(R_{Sender}) \stackrel{?}{=} R_{n-1,l}$


%Spalte rechts mit Rank_{sender}

% 1
$dec _{c_{2}} (c_{1}) = R_{1, l}$
\newline\vspace{0.03cm}
$h^{l-Rank_{sender}}(R_{sender}) \stackrel{?}{=} R_{1,l}$

% 2
$dec _{c_{3}} (c_{2}) = R_{2, l}$
\newline
$h^{l-Rank_{sender}}(R_{sender}) \stackrel{?}{=} R_{2,l}$

% 3
$dec _{c_{4}} (c_{3}) = R_{3, l}$
\newline
$h^{l-Rank_{sender}}(R_{sender}) \stackrel{?}{=} R_{2,l}$

% n-1
$dec _{R_{n,l}} (c_{n-1}) = R_{n-1, l}$
\newline
$h^{l-Rank_{sender}}(R_{sender}) \stackrel{?}{=} R_{n-1,l}$






% n -1
\begin{tiny}
$\textrm{verify:}  V_{(n-1)}  \textrm{\,{\&}\,} $
\vspace{0.03cm}

\hspace{0.4cm} $\textrm{\textrm{MAC}}_{V_{(n-1)}}(R_{(n-1), l}) $
\end{tiny}
\vspace{0.03cm}

$dec _{R_{n,l}} (c_{(n-1)}) = R_{(n-1), l}$
\vspace{0.15cm}

% Hashvalue left

$h(V_{1})$ 
 
\bigskip 

$h(V_{2})$ 

\bigskip 

$h(V_{3})$ 

\bigskip 

$h(V_{4})$ 

\bigskip 

$h(V_{(n-1)})$ 

\bigskip $h(h(x))$

\vspace{0.15cm}

%Version number left

$V_{0}$ 

\bigskip 

$V_{1}$ 

\bigskip 

$V_{2}$ 

\bigskip 

$V_{3}$ 

\bigskip 

$V_{(n-1)}$


==> 02_tables/01_encryptChain.tex <==
\begin{table}
 \centering
 % \begin{minipage}[b]{.5\linewidth} % [b] => Ausrichtung an \caption
\begin{tabular}{|  c  | }
\hline
 $\textrm{root creates encryption chain}$ \\
\hline \hline
$encrypt(DATA, KEY) = \textrm{encrypted data}$ \\
\hline
$encrypt(V_{5}R_{mrh}, V_{4}R_{mrh}) = MRH_{1}$ \\
\hline
$encrypt(MRH_{1}, V_{3}R_{mrh}) = MRH_{2}$ \\
\hline
$encrypt(MRH_{2}, V_{2}R_{mrh}) = MRH_{3}$ \\
\hline
$encrypt(MRH_{3}, V_{1}R_{mrh}) = MRH_{4}$ \\
\hline
\end{tabular}
\vspace{1mm}\\
  \caption{}
    \label{tab:encChain}
%  \end{minipage}
  \end{table}


==> 02_tables/02_veraAddition.tex <==

\setlength{\fcwidth}{2cm}
\begin{table}
  \centering
    \begin{tabular}{l l l}
    \toprule
        \multicolumn{2}{c}{Hash Chains} & \multicolumn{1}{c}{Encryption Chain}\\
        \cmidrule(lr){1-2} \cmidrule(lr){3-3}
        \multicolumn{1}{l}{Version Element} & \multicolumn{1}{l}{Rank Element} & \multicolumn{1}{l}{Rank Element}\\
        \multicolumn{1}{l}{$V_{i} = h(V_{i+1})$} & \multicolumn{1}{l}{$R_{i,j} = h(R_{i,j-1})$} & \multicolumn{1}{l}{$c_i=enc_{c_{i+1}}(R_{i,l})$}\\
        %\hline \hline
        \midrule
        \multirow{4}{\fcwidth}{$V_{n} = h^1(r)$} & $R_{n,l} = h^{l+1}(x_n)$ & {$c_n = R_{n,l}$} \\ 
        &  {\ldots} & \\
         & $R_{n,1} = h^2(x_n)$ & \\ 
         & $R_{n,0} = h^1(x_n)$ & \\ 

        \midrule

        \multirow{3}{\fcwidth}{$V_{n-1} = h^2(r)$} &  {$R_{n-1,l} = h^{l+1}(x_{n-1})$}  & {$c_{n-1} = enc_{c_{n}}(R_{n-1,l})$} \\ 
        &  {\ldots} & \\
        &  {$R_{n-1,0} = h^1(x_{n-1})$} & \\ 

        \midrule

        \ldots &  \ldots & \dots \\

        \midrule

        \multirow{4}{\fcwidth}{$V_{1} = h^{n-1}(r)$} & {$R_{1,l} = h^{l+1}(x_1)$} & {$c_1 = enc_{c_2}(R_{1,l})$}  \\
        &  {\ldots} & \\
        & {$R_{1,0} = h^1(x_1)$} &   \\

        \midrule

        \multirow{4}{\fcwidth}{$V_{0} = h^n(r)$} & {$R_{0,l} = h^{l+1}(x_0)$} & {$c_0 = enc_{c_1}(R_{0,l})$}  \\
         &  {\ldots}  & \\
         & {$R_{0,0} = h^1(x_0)$}  &   \\
      \bottomrule
    \end{tabular}
    %\caption{Creation of the Hash Chains and the Encryption Chain ($r$ and $x_i$ are random numbers, $h(\cdot)$ denotes a hash function, $enc_k(\cdot)$ an encryption function with key $k$)}
    \caption{Creation of the Hash Chains and the Encryption Chain}
    \label{tab:veraAdd}
\end{table}




==> 02_tables/04_TRAIL_filter_construction.tex <==
\begin{table}[htb]
\centering%
\begin{tabular}{c c c }
  \toprule
  Child Node  & Nonce  & Bloom Filter Array \\
 \midrule
  &&\\
  $N_{l,1}$ & $\eta_{l,1}$ & $A_1:\{v_1,\dots, v_n\}$ \\ 
   \vdots& \vdots & \vdots \\ 
  $N_{l,k}$ & $\eta_{l,k}$ & $A_k:\{v_1,\dots, v_n\}$ \\
  &&\\
  \midrule
  $B$ & $v_B:=\cup(\eta_{l,1},\dots, \eta_{l,k})$ & $B:\{ v_B, \cup(A_1,\dots, A_k)\}$ \\
	& &\\
  \bottomrule
\end{tabular}
\caption{View of a parent node of leaves: \textnormal{The received Bloom filter arrays $A_1 \ldots A_k$ are united into the new array $B$ starting at its 2nd index. $B(1)$ holds the united received nonces $\eta_{l,1} \ldots. \eta_{l,k}$ in a newly created filter $v_B$.} }

\end{table}

 

